AgentOhana: Design Unified Data and Training Pipeline for Effective Agent Learning

Autonomous agents powered by large language models (LLMs) have garnered significant research attention. However, fully harnessing the potential of LLMs for agent-based tasks presents inherent challenges due to the heterogeneous nature of diverse data sources featuring multi-turn trajectories. In this paper, we introduce \textbf{AgentOhana} as a comprehensive solution to address these challenges. \textit{AgentOhana} aggregates agent trajectories from distinct environments, spanning a wide array of scenarios. It meticulously standardizes and unifies these trajectories into a consistent format, streamlining the creation of a generic data loader optimized for agent training. Leveraging the data unification, our training pipeline maintains equilibrium across different data sources and preserves independent randomness across devices during dataset partitioning and model training. Additionally, we present \textbf{xLAM-v0.1}, a large action model tailored for AI agents, which demonstrates exceptional performance across various benchmarks. Begin the exploration at \url{https://github.com/SalesforceAIResearch/xLAM}.

==> auto_agent.tex <==
\subsection{Augmented Language Agent Architecture}
% From search to learn, from earlier to later
% Add the applications like, HuggingGPT, BabyAGI as applications of the proposed agent structure
The completion of a complex task typically entails multiple stages. An agent must possess an understanding of these stages and plan accordingly. Chain-of-Thoughts, also known as CoT~\citep{wei2022chain}, is a groundbreaking work that prompts the agent to deconstruct challenging reasoning tasks into smaller, more manageable steps. On the other hand, ReAct~\citep{yao2023react} proposes leveraging this aptitude for reasoning and action within Language and Learning Models (LLMs) to foster interactive engagement with the environment, such as utilizing the Wikipedia search API, by mapping observations to the generation of reasoning and action traces or API calls in natural language. This agent architecture has given rise to various applications, including HuggingGPT~\citep{shen2023hugginggpt}, Generative Agents~\citep{park2023generative}, WebGPT~\citep{nakano2021webgpt}, AutoGPT~\citep{autogpt23}, BabyAGI~\citep{babyagi23}, and Langchain~\citep{langchain23}. 

However, these approaches neglect to incorporate valuable feedback, such as environment rewards, to enhance the agent's behaviors, resulting in performances that rely solely on the quality of the pre-trained Language and Learning Model (LLM). Self-refine~\citep{madaan2023learning} tackles this limitation by employing a single LLM as a generator, refiner, and provider of feedback, enabling iterative refinement of outputs. However, it is not specifically tailored for real-world task-based interaction with the environment. On the other hand, REX~\citep{murthy2023rex} and RAP~\citep{hao2023reasoning} repurpose the LLM to function as both a comprehensive world model and a reasoning agent. They incorporate Monte Carlo Tree Search for strategic exploration within the vast realm of reasoning with environment rewards. This approach facilitates effective navigation and decision-making in intricate domains. \citet{shinn2023reflexion} presents Reflexion, a framework that equips agents with dynamic memory and self-reflection capabilities, enhancing their reasoning skills. Self-reflection plays a pivotal role, allowing autonomous agents to iteratively refine past actions, make improvements, and prevent repetitive errors. Recently, \citet{yao2023retroformer} proposes a framework, namely Retroformer, which leverages policy gradient optimization to align the agent's behaviors with environment-specific rewards by learning a plug-in retrospective language model.

==> webshop_perf.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}


